Cutting Polygons into Small Pieces with Chords: Laser-Based Localization

Motivated by indoor localization by tripwire lasers, we study the problem of cutting a polygon into small-size pieces, using the chords of the polygon. Several versions are considered, depending on the definition of the "size" of a piece. In particular, we consider the area, the diameter, and the radius of the largest inscribed circle as a measure of the size of a piece. We also consider different objectives, either minimizing the maximum size of a piece for a given number of chords, or minimizing the number of chords that achieve a given size threshold for the pieces. We give hardness results for polygons with holes and approximation algorithms for multiple variants of the problem.

==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file


==> README <==
The mathtools bundle
=============
Morten Hoegholm (c) 2002-2011
Lars Madsen     (c) 2012-
email: daleif@math.au.dk
License: LaTeX Project Public License

The files in the mathtools bundle are:
    mhsetup.dtx
    mathtools.dtx
    empheq.dtx
and derived files. The derived files of each .dtx-file are listed
at the top of the respective .dtx-file.


INSTALLATION
============
Running TeX on each dtx file extracts the runtime files. See the dtx
files for details.

DESCRIPTION
===========


mathtools
=========

The mathtools package provides many useful tools for mathematical
typesetting. It is based on amsmath and fixes various deficiencies
of amsmath and standard LaTeX. It provides:
  -- Extensible symbols, such as brackets, arrows, harpoons, etc.
  -- Various symbols such as \coloneqq (:=).
  -- Easy creation of new tag forms.
  -- Showing only the referenced equations.
  -- Extensible arrows, harpoons and hookarrows.
  -- Starred versions of the amsmath matrix environments for
     specifying the column alignment.
  -- More building blocks: multlined, cases-like environments, new
     gathered environments.
  -- Math versions of \makebox, \llap, \rlap etc.
  -- Cramped math styles.
  -- Macro generators.
  -- and more...

mathtools requires mhsetup.

empheq
======

The empheq package is a visual markup extension designed to
function on top of amsmath. It features:
  -- Boxing multi line math displays while leaving equation
     numbers untouched at the margin. Any kind of box will do.
  -- Making the ntheorem package place end-of-theorem markers
     perfectly.
  -- Placing arbitrary material on either side of math displays.
     This includes delimiters that automatically scale to the
     correct size.

empheq requires mathtools.


mhsetup
=======

The mhsetup package defines various programming tools needed by
both empheq and mathtools. The syntax is the same as for expl3, 
but there is no code overlap (anymore as of May 2017).
In the future, most of these tools will probably be an integral part of LaTeX3 (they were). 


BUG REPORTS
===========

The bundle is maintained by:

  Morten H\o gholm  
  Lars Madsen <daleif@math.au.dk>
  

Please report bugs to daleif@math.au.dk

===========
This README file was last revised 2017/05/24.


==> circle-old.tex <==
\section{$O(\log\opt)$-approximation for \mlc}\label{sec:circle}
This section considers the radius of the largest inscribed circle as the measure of cell size; in particular, in \mlc the goal is to split the polygon \P (which may contain holes) into pieces so that no piece contains a disk of radius 1. We give an $O(\log\opt)$-approximation algorithm for \mlc based on reducing the problem to SetCover.
The following reformulation is crucial for the approximation algorithm:
\begin{observation}\label{obs:reformulation}
A set of lasers splits \P into pieces of in-circle radius at most 1 iff every unit disk that lies inside \P is hit by a laser.
\end{observation}

\begin{theorem}\label{thm:apxcircle}
For a polygon \P with $n$ vertices (possibly with holes),
\mlc admits an $O(\log\opt)$-approximation in time polynomial in $n$ and $\area(P)$.
%\val{changed \diam to \area -- of course, poly in one is poly in the other, but here the time directly depends on the area}
\end{theorem}
\begin{proof}
Let $\P^{-1}$ be the set is points in \P that are further than 1 unit from the boundary of the polygon (i.e., the set of centers of unit disks contained inside \P) and let $\P'$ be the Minkowski sum of $\P^{-1}$ and unit disk (i.e., the points of the polygon that can be covered by a unit disk contained in \P).
In principle both $\P^{-1}$ and $\P'$ can either be built from the medial axis of \P (the medial axis consists from a polynomial number of constant-complexity elementary pieces---segments, circular and parabolic arcs; therefore the boundary of $\P^{-1}$ also does, so in polynomial time one can build the full arrangement of the Minkowski sums of the pieces with the unit disk -- and hence their union) or computed by rolling unit disk along the boundary of \P. However, in our algorithm we do not have to build either $\P^{-1}$ or $\P'$ explicitly. All we need is to know whether a given square can be covered by a unit disk fully lying inside \P. This can be accomplished by overlaying the square with the Voronoi diagram of \e{features} (vertices and edges) of \P and then checking whether there exists a point of the square further than 1 from the boundary of \P (we do not optimize the running times of our algorithms, focusing only on polynomial time).

Specifically, we take an infinite square grid with pixel size (i.e., side length) $1/\sqrt2$ (the orientation and the horizontal and vertical shifts of the grid do not matter), and keep only the pixels (i.e., grid cells) that lie fully inside $\P'$ (Fig.~\ref{fig:apxcircle}). We denote the set of these pixels by $G$; clearly their number is $O(\area(P))$.

Consider the instance of SetCover $(G,\cal L)$ in which $G$ is the universe and every set in $\cal L$ is formed by a subset of pixels intersected by a chord of \P. Since a 3x3 square of pixels cannot be shattered by $\cal L$, the VC dimensions of the set system $G,\cal L$ is constant. Hence, by Sauer--Shelah's Lemma \cite{sauer,shelah}, $|\cal L|$ is polynomial in $|G|$ (in fact, to define the subsets in $\cal L$, it suffices to consider the chords that pass through two vertices of the pixels or vertices of \P -- this can be seen by shifting any chord, while it still goes through the same set of pixels, until it hits a vertex of a pixel or a vertex of \P and then rotating the chord until the next hit)
and we can find an $O(\log\opt)$-approximate solution to the SetCover in time polynomial in $n$ and $\area(P)$ \cite{BG} .
%(the number of sets in $\cal L$ is polynomial in $n$ and $\area(\P)$, and all the sets can be explicitly computed in polynomial time).

We now argue that an $O(\log\opt)$-approximate solution to the SetCover problem is also an $O(\log\opt)$-approximate solution to \mlc. First, since any unit disk fully contains at least one pixel from the grid (the pixels have unit diagonals), the solution is feasible. The approximation factor follows from the fact that any solution (a set of lasers) $L$ to \mlc can be converted to a solution to the SetCover of size $O(|L|)$ by placing a constant number of evenly spaced copies of every laser $\ell\in L$, running parallel to $\ell$ symmetrically on both sides of the laser (Fig.~\ref{fig:apxcircle}, middle).
\csaba{It is unclear how the copies are placed: Each laser in $L$ is a chord of $P$, and a parallel line might intersect the boundary of $P$ several times. Some technicality is missing...}
\val{It seems there can be polygons in which the number of chords to intersect all green pixels is much larger than the number of chords to intersect all unit disks (Fig.~\ref{fig:error})}
The width of the strip covered by the copies (i.e., the distance between the outermost copies) is 4 and the distance between consecutive copies is a constant $d$ defined below. By definition of $\P'$, the center of every pixel $g\in G$ is contained in a unit disk $D$ lying fully inside \P. Since $D$ is intersected by a laser $\ell\in L$, the width-4 strip of lasers, corresponding to $\ell$ covers $D$. In particular, any diameter-$d$ disk lying fully inside $D$ intersects at least one laser from the strip. But the intersection $g\cap D$ does contain such a disk (Fig.~\ref{fig:apxcircle}, right); hence, the intersection (and hence $g$) is intersected by a laser, implying that the optimal solutions to \mlc and the SetCover differ by a constant factor.
Overall, an $O(\log\opt)$-approximate solution to the SetCover is also one for \mlc.
\end{proof}

\begin{figure}\centering\includegraphics[width=.5\columnwidth]{error}\caption{The squares do not belong to a ragular grid, but still...}\label{fig:error}\end{figure}

\begin{figure}[htbp]
\centering\includegraphics{apxcircle}\hfil\includegraphics[width=.3\columnwidth]{gg.png}\caption{Left: %$\P^{-1}$ (blue) is curved out of \P (black) by a unit disk rolling along the polygon boundary.
$\P'$, defined by unit disk rolling along $\partial\P$ (black), may have multiple connected components bounded by edges of \P and unit-circle arcs (red). Sets of pixels (green) are intersected by chords (blue) pinned on vertices of pixels or \P. Middle: Copies (blue dashed) of a laser in $L$ (blue) intersect any width-$d$ set lying inside unit disk $D$ (black), in particular, the intersection of the pixel and the disk. Right: Zoom-in on the intersection of $g$ and $D$ -- a snapshot of the GeoGebra applet https://www.geogebra.org/m/ffc5haxq. The intersection is smallest when the center $a$ of $g$ is on the boundary of $D$, so assume that the center $c$ of $D$ is on a unit circle (dotted) centered at $a$. W.l.o.g.\ $c$ is NE of $a$, i.e., in the first quadrant w.r.t.\ $a$ (the extreme positions of $D$ are dashed). The disk of radius $d=1/8$ (green) centered on the midpoint of the half-diagonal $ab$ of $g$ is contained in $g$ and is contained in the intersection of the two extreme positions of $D$, and hence is contained $D$ no matter where $c$ is (this can also be seen by moving $c$ in the applet\csaba{We shouldn't suggest that experiments with an  applet constitute a proof.}).
}\label{fig:apxcircle}\end{figure}

\rathish{Based on my discussion with Joe in last week, we formulated the set cover where we hit the disks themselves. We used two types of disks --- 1) red disks, that are adjacent to the polygon boundary (including holes) 2) blue disks, which is a grid of disks inside of the polygon. A red and a blue disk may overlap. We need to hit all the red and blue disks. Note that we said grid of disk, we are not laying out squares to be hit. Once we get the set-cover solution we replicate the lasers on both sides.}

\csaba{I don't understand how the red and blue disks are defined. Perhaps one can get a bicriteria solution using a grid of disks, and use it for a constant-factor approximation?}

\val{will try to write bi-criteria}

\subsection{Bi-criteria (1+\eps,$O(\log\opt)$)-approximation for incircle}\val{Replace the section with this if this is ok (need fig?)}

This section considers the radius of the largest inscribed circle as the measure of cell size. Let \opt denote the minimum number of lasers required to split a polygon \P (possibly with holes) into pieces so that no piece contains a disk of radius 1; abusing the notation, we will use \opt both for the solution and the number of lasers in it. We will place $O(\opt\log\opt)$ lasers that split \P into pieces with incircle radius at most 1+\eps. The approximation is based on reducing the problem to SetCover and is inspired by Baker's grid shifting technique \cite{baker}.
The following reformulation is crucial for the approximation algorithm:
\begin{observation}\label{obs:reformulation}A set of lasers splits \P into pieces of in-circle radius at most 1 iff every unit disk that lies inside \P is hit by a laser.\end{observation}

\begin{theorem}\label{thm:apxcircle}
$O(\opt\log\opt)$ lasers splitting \P into parts with incircle radius at most 1+\eps can be found in time polynomial in $n,\frac1\eps$ and $\area(P)$ \rathish{where $\epsilon$>0?}.
\end{theorem}
\begin{proof}%Let $D(c,r)$ denote the radius-$r$ disk centered at $c$.
Let $P'$ be the "erosion" of \P by 1+\eps, i.e., the set of points in \P that are further than 1+\eps from $\partial\P$, or equivalently, the set of centers of radius-(1+\eps) disks that are fully contained inside \P. The set $\P'$ (which may have more than 1 connected component) can either be computed from the medial axis of \P %(the medial axis consists from a polynomial number of constant-complexity elementary pieces---segments, circular and parabolic arcs; therefore the boundary of $\P'$ also does)
or traced by rolling disks along the boundary of \P.
We place an \eps-dense set of points in $P'$, i.e., a set $C:\forall p\in P'\exists c\in C:|pc|\le\eps$. The set $C$ can be built from a maximal packing of radius-\eps/2 disks or computed iteratively by placing new points at the vertices of the Voronoi diagram of existing points as long as the empty disk at the Voronoi vertex has radius larger than \eps. Let $G$ be the set of unit disks centered on points in $C$. \rathish{Please check that if a figure wold help the construction of set $C$ or $G$}

Consider the instance of SetCover $(G,\cal L)$ in which $G$ is the universe and every set in $\cal L$ is formed by a subset of disks intersected by a chord of \P. Since there exists a constant-size set of disks that cannot be shattered by $\cal L$, the VC dimensions of the set system $(G,\cal L)$ is constant \rathish{Why it is true that there exists a constant-size set of disks that cannot be shattered by $\cal L$?}. Hence, by Sauer--Shelah's Lemma \cite{sauer,shelah}, $|\cal L|$ is polynomial in $|G|$ (in fact, to define the subsets in $\cal L$, it suffices to consider the chords bitangent to two disks or vertices of \P -- this can be seen by shifting any chord, while it still goes through the same set of disks, until it becomes tangent to a disk or a vertex of \P and then rotating the chord until the next tangency)
and we can find an $O(\log\opt_{SC})$-approximate solution to the SetCover in time polynomial in $|G|$ (and $|\cal L|$, which is polynomial in $n$ and $\area(P)/\eps$ \cite{BG} (here $\opt_{SC}$ is the size of the optimal solution to the SetCover).

Consider now any disk $D(c,1+\eps)\subset\P$ \rathish{Is this a standard notation to specify the center and the radius of a circle?} that has to be hit in a feasible cutting of \P into pieces with in-circles at most 1+\eps ($c\in P'$). Since $C$ is \eps-dense in $P'$, there exists a point $g\in G$ with $|cg|\le\eps$, implying that $D(g,1)\subset D(c,1+\eps)$. Since the unit disk $D(g,1)$ is hit by a chord in our solution to the SetCover, $D(c,1+\eps)$ is also hit; hence our solution is a feasible cutting into pieces of size 1+\eps. As for the approximation factor, since $C\subset P'$, all disks $G$ are inside \P and, by Observation~\ref{obs:reformulation}, have to be hit by \opt. Thus, $\opt\ge\opt_{SC}$ and we placed $O(\opt_{SC}\log\opt_{SC})=O(\opt\log\opt)$ lasers.\end{proof}


==> conclusion.tex <==
\section{Conclusion}
\val{remove for the submission?}



==> convex-cell.tex <==
\section{Decomposition into Convex Cells}
\label{sec:convex}

We first address the problems with the added constraint that each induced cell is required to be convex.

\subsection{MinLaser-ConvexDiameter}

For the problem MinLaser-ConvexDiameter on a simple polygon, we consider a threshold $\delta$ given as the maximum diameter of each piece and minimize the number of lasers needed.
As an appetizer, we start from the case when $P$ is a convex polygon. Then we look at the general case.

\subsubsection{Convex Polygons}

Divide the perimeter of the simple convex polygon $P$ evenly with separation of $\delta/\sqrt{2}$. The total number of points is $\frac{\per(P)}{\delta/\sqrt{2}}$. We put two lasers, one horizontal and one vertical on each point. These lasers partition the polygon into $m$ pieces. Notice that each piece is bounded within a rectangle of side length at most $\delta/\sqrt{2}$.
Let $d$ be the maximum diameter of any piece, $d \leq  \delta$.

\begin{theorem}
The above algorithm solves the  MinLaser-ConvexDiameter on a convex polygon with an approximation factor of $4\sqrt{2}\pi$.
\end{theorem}
\begin{proof}
We would like to argue a lower bound on the number of lasers needed for the optimal solution.
Consider the boundary of the convex polygon $P$. We argue that any part of the boundary of length at least $\pi\delta$ must be cut by at least one laser -- otherwise, the diameter of this piece exceeds $\delta$.  Therefore any feasible solution (including the optimal) needs to use at least $\frac{\per(P)}{4\pi\delta}$ lasers---neighboring chains may share one laser cut and one laser cuts two places on the boundary of $P$.  Our solution uses at most $\frac{2\per(P)}{\delta/\sqrt{2}}$ lasers. Thus the approximation could be derived as at most $4\sqrt{2}\pi$.
%Time Complexity : $O(\frac{\per(P)}{\delta})$
\end{proof}

\subsubsection{Simple Polygons}

We show that this problem admits an $(8\sqrt{2}\pi+4)$-approximation by placing two lasers orthogonally on the following set of points: (1) each reflex vertex of the polygon; (2) points evenly placed on the perimeter of the polygon with separation of $\delta/\sqrt{2}$.

\begin{theorem}
Given a threshold $\delta$ on the maximum diameter of each piece, we can cut a given simple polygon into pieces by using lasers whose number is at most a factor $8\sqrt{2}\pi+4$ of the minimum possible.
\end{theorem}
\begin{proof}
We first consider finding lower bounds on the number of lasers needed for cutting the polygon into convex pieces of diameter at most $\delta$.

If there is a chain along the polygon boundary with length greater than $\pi \delta$ but has maximum diameter at most $\delta$, there must be a reflex vertex in that chain. As each piece has to be convex, there must be a laser which intersects a chain with length $\pi \delta$ either because its diameter would be more than $\delta$ otherwise, or because the chain has a reflex vertex. Suppose $P$ has perimeter $\per(P)$, there are $\per(P)/(\pi \delta)$ chains of length $\pi \delta$. Each chain is cut at least once by some laser. Note that each laser only hits two points on the polygon boundary. Thus one lower bound for the optimal solution (denoted by OPT) could be derived as the number of lasers needed to hit all these chains. Let this lower bound be denoted by $C_{1}^{*}$. We have,
	\begin{equation}
	C_{1}^{*}= \frac{\per(P)}{4\pi \delta} \leq \opt.
	\end{equation}
\jie{since two neighboring chains share one endpoint, thus the above lower bound shall be $\per(P)/(4 \pi \delta)$ instead of $\per(P)/(2 \pi \delta)$.}
\val{Maybe we may consider chains of length $\pi+\eps$, e.g., for just "small enough" $\eps$ similarly to Section~\ref{sec:minLaser-Diameter}, or specifically for $\eps$ small enough to have the same rounding (we may need to round carefully anyway -- the lower bound has floor while apx has ceiling)? Then every chain has to be hit in the interior, and so 1 laser can hit only 2 chains (and then the lower bound is $\per(P)/(2\pi)$}

Further, if there are $r$ reflex vertices, any solution must use at least $r/2$ lasers to remove these reflex vertices. This gives another lower bound
	\begin{equation}
	C_{2}^{*}= r/2 \leq OPT.
	\end{equation}
	
Now we are ready to prove the approximation ratio of our algorithm. First we place two lasers along the polygon boundary for every segment of length $\delta/\sqrt{2}$. This amounts to $2\sqrt{2} \cdot \per(P)/\delta = 8\sqrt{2}\pi C_{1}^{*}\leq 8\sqrt{2}\pi \cdot OPT$.
%	\begin{equation}
%	\begin{aligned}
%		C_{1} &\leq  \frac{2\sqrt{2}\per(P)}{\delta} \\
%		 &\leq 4\sqrt{2}\pi C_{1}^{*}
%	\end{aligned}
%	\end{equation}
Second, we place two lasers at each reflex vertex. This amounts to $2r= 4C_{2}^{*}\leq  4 OPT$.	
%	\begin{equation}
%	\begin{aligned}
%	C_{2} &\leq  2R \\
%	&\leq 4C_{2}^{*}
%	\end{aligned}
%	\end{equation}
This gives an approximation ratio of $8\sqrt{2}\pi +4$.	
%	\begin{equation}
%	\begin{aligned}
%	C &\leq C_{1} + C_{2} \\
%	  &\leq (4\sqrt{2}\pi C_{1}^{*} + 4C_{2}^{*}) \\
%	  &\leq 4\sqrt{2}\pi(2.max(C_{1}^{*},C_{2}^{*})) \\
%	  &\leq 8\sqrt{2}\pi C^{*}
%	\end{aligned}
%	\end{equation}
\end{proof}
%Time Complexity : $O(n+\frac{\per(P)}{\delta})$ where $n$ is number of reflex vertices. 


\subsection{MinLaser-ConvexArea}

We present an algorithm for a general simple polygon with an $O(\log r)$-approximation, where $r$ is the number of reflex vertices of the given polygon $P$.

We use the convex subdivision of $P$ from Lemma~\ref{lem:CxDecomp} for positioning lasers in $P$ as follows.
First, for each edge $e$ in the convex subdivision of $P$, we place a laser at the chord of $P$ that contains $e$. Since Hershberger-Suri triangulation has $O(r)$ triangles, this requires $O(r)$ lasers.
Let $T$ denote the convex regions of the subdivisions whose area is more than $\delta$.
For every region $t\in T$, we use at most $O(\sqrt{\area(t)/\delta})$ lasers to subdivide
it into regions of area at most $\delta$, by Lemma~\ref{lem:Convex-ConvexArea}.

\begin{theorem}
There is an algorithm that finds an $O(\log r)$-approximation for MinLaser-ConvexArea for a simple polygon $P$ with $n$ vertices, $r$ of which are reflex, in $O(n\log n)$ time.
%	There is an $O(\log r)$-approximation algorithm for MinLaser-ConvexArea for simple polygons.
\end{theorem}
\begin{proof}
Let $P=(v_1,\ldots v_n)$ be a simple polygon, and let $\opt$ denote the minimum number of lasers that
can subdivide $P$ into convex regions of area at most $\delta$. In an optimal solution, each reflex vertex of $P$ is incident to at least one laser, and each laser is incident to at most two vertices of $P$. Consequently, we have $\opt\geq r/2$, where $r$ is the number of reflex vertices.
That is, the number of lasers placed along the edges of the Hershberger-Suri triangulation of $P$ is $O(r)=O(\opt)$.

Next, we consider the lasers used for subdividing the convex regions in $T$, whose area is more than $\delta$.
Each region $t\in T$ intersects at least $\Omega(\sqrt{\area(t)/\delta})$ lasers in an optimal solution (by Lemma~\ref{lem:Convex-ConvexArea});
and conversely each laser of an optimal solution intersects $O(\log r)$ regions in $T$. Consequently,
the number of lasers we use is $\sum_{t\in T}\sqrt{\area(t)/\delta}\leq O(\opt \, \log r)$.

Overall, our algorithm uses $O(r+ \sum_{t\in T}\sqrt{\area(t)/\delta}) =O(\opt+\opt\, \log r)=\opt\, O(\log r)$ lasers.
\end{proof}

\subsection{$k$-Laser-MinMaxConvexArea}
%Notes on Possible $O(1)$-Approximation for Partitioning to Minimize Maximum Area in Convex Partition}

% pasted in by Estie:

We start with the case when $P$ is a convex polygon.
\begin{theorem}
The $k$-Laser-MinMaxConvexArea problem can be approximated by a constant factor for a convex polygon $P$.
\end{theorem}
\begin{proof}
First let's look at the special case when $P$ is a rectangle. We claim that by placing $k/2$ lasers equally spaced vertically and the remaining $k/2$ equally spaced horizontally we have a constant factor approximation to the optimal. A lower bound on OPT is the area of the rectangle divided by the maximum possible number of faces in an arrangement of $k$ lines, namely ${k \choose 2}+k+1=O(k^2)$.  Our placement of lines yields $(k/2 +1)^2$ equally sized regions.
%
%Problem 1:
%Given a rectangle and $k$ lasers, place them to minimize the area of
%the largest face.
%
%Claim: Placing $k/2$ lasers equally spaced vertically and the remaining $k/2$ equally spaced horizontally yields a constant factor approximation.
%Proof: A lower bound on OPT is the area of the rectangle divided by the maximum possible number of faces in an arrangement of $k$ lines, namely ${k \choose 2}+k+1=O(k^2)$. Our placement of lines yields $(k/2 +1)^2$ equally sized regions.

%Problem 2:
%Given a convex region, place $k$ lasers to minimize the
%maximum area of a face.
%
%Claim: We can approximate this with $O(1)$ factor.
%
%Proof: Find the diameter of the convex region and build a bounding
%rectangle with that as the horizontal direction. Now apply the
%previous placement to the bounding rectangle.  Note -- the area of the
%bounding rectangle is at most twice the area of the convex region.

For a convex polygon $P$, we can find its diameter $ab$ and build a smallest bounding
rectangle $D$ with $ab$ as the horizontal direction. Now we apply the earlier solution for the bounding rectangle $D$. Notice that the area of the bounding rectangle $D$ is at most twice the area of the convex region. %\jie{More explanation on this sentence?}
To see why, consider the contact points at the top/bottom of the bounding rectangle, named $c, d$ respectively. By convexity, the area of the polygon $P$ is at least the sum of the area of the two triangles $\triangle abc, \triangle abd$, which is half of the area of the bounding rectangle.
Therefore the solution gives an $O(1)$ approximation of the optimal.
\end{proof}

Problem 3: Given a simple polygon, place $k$ lasers to minimize the
maximum area of a face.

\joe{Estie withdraws this claim (the convex pieces cannot be handled separately, as lasers go through the chords that partition into convex pieces).}

Claim: This can also be apx with an $O(1)$ factor??

Idea of proof: Partition the polygon into the minimum (?) number of convex pieces, $P_1$, ..., $P_m$. We now decide how many lasers $k_i$ to allocate to each piece $P_i$ based on its area, with the goal to minimize the maximum of area($P_i$)/($k_i/2+1)^2$  with $\sum_i k_i=k$.

\joe{% Joe adds:
Note that, knowing we will use the bounding rectangle method to
partition a convex piece, we can use dynamic programming to obtain an
optimal partition into convex pieces, minimizing the maximum area of a
face obtained by using this method, minimizing over all possible
convex partitions.}



==> exact-alg.tex <==
\section{Exact Algorithms}

\Att{What about rectangles or convex polygons, with axis parallel cuts?}



==> hardness-short.tex <==
\section{Hardness in Polygons with Holes}\label{sec:hardness-short}
We show that for all three measures (area, diameter, the radius of the largest inscribed circle) it is NP-hard to decide whether a given polygon \P \emph{with holes} can be divided into pieces of small measure using a given number of lasers, both for unrestricted-orientation and axis-aligned lasers. %; and for the case where the resulting pieces are constrained to be convex.

We prove hardness by reduction from the 3SAT problem. Our polynomial-time reduction is similar to previous reductions for line cover problems, which are geometric variants of set cover~\cite{LangermanM05}. In particular, Megiddo and Tamir~\cite{MegiddoT82} proved that the \textsc{LineCover} problem is NP-complete: Given $n$ points in the plane and an integer $k$, decide whether the points can be covered by $k$ lines. Hassin and Megiddo~\cite{HassinM91} proved hardness for \textsc{MinimumHittingHorizontalUnitSegments} problem: Given $n$ horizontal line segments in the plane, each of unit length, and an integer $k$, decide whether there exists a set of $k$ axis-parallel lines that intersects all $n$ segments. Our reduction is based on the idea of Hassin and Megiddo, but requires highly non-trivial adjustments to generate a subdivision of a polygon. All proofs are in Appendix~\ref{sec:hardness-full}. We remark that tractability in the case of simple polygons remains open.


==> macros.tex <==
\usepackage{amsmath,amssymb,amsthm}
\usepackage{graphicx}
\usepackage[mathscr]{euscript}
\usepackage{tikz}
\usetikzlibrary{trees,arrows,automata}
\usetikzlibrary{shapes.geometric} % for oval nodes
\usetikzlibrary{shadows,fadings}
\usepackage{wrapfig}   % for wrapfig function
\usepackage{stmaryrd} % for llceil function
\usepackage{url}
\usepackage{pifont}
\usepackage{lipsum}
\usetikzlibrary{arrows,shapes,positioning,shadows,trees}
\usepackage{multirow}
%---- TCOLORBOX -----
\usepackage{tcolorbox}
\tcbuselibrary{skins}
%----- TABLE COLOR -----
\usepackage{environ}
\usepackage{colortbl}
\usepackage{hhline}
\usepackage{rotating}
\usepackage{array}
\usepackage{libertine}
\usepackage{enumitem}
\usepackage{mdframed}

\newcommand{\hide}[1]{}
%\newtheorem{property}{Property}
%\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{question}{Question}[section]
\newtheorem{rules}{Rule}
\newcommand{\floor}[1]      {\left\lfloor #1 \right\rfloor}
\newcommand{\highlight}[1]{\textit{#1}}
\newcommand{\highlighttitle}[1]{\textbf{#1}}
\newcommand\pa[1]{\ensuremath{\left(#1\right)}}

\newcommand{\DPTab}{C}

\newcommand{\cnote}[2]{%
  \ifnotes
    {\marginpar{\color{#1}\scriptsize \sf \raggedright{#2}}}%
%    {\marginpar{\color{#1}\small\raggedright\parbox[t]{\columnwidth}{#2}}}
  \fi}

\definecolor{gray}{rgb}{0.3,0.3,0.3}
\definecolor{orange}{rgb}{1,0.3,0}
\newcommand{\rezaulnote}[1]{\cnote{red}{Rezaul: #1}}

\def\comment#1{\hfill{\color{gray}{$\left\{\textrm{{\em{#1}}}\right\}$}}}
\def\lcomment#1{\hfill{\color{gray}{$\left\{\textrm{{\em{#1}}}\right.$}}}
\def\rcomment#1{\hfill{\color{gray}{$\left.\textrm{{\em{#1}}}\right\}$}}}
\def\fcomment#1{\hfill{\color{gray}{$\textrm{{\em{#1}}}$}}}
\def\func#1{\textrm{\bf{\sc{#1}}}}
\def\funcbf#1{\textrm{\textbf{\textsc{#1}}}}
\def\F#1#2{\func{${#1}_{#2}$}}
\def\L#1#2{\func{${#1}_{loop\text{-}#2}$}}
\newcommand{\tim}[1]{\textbf{TIME: \{} #1 \textbf{\}}}
\newcommand{\oq}{\mbox{``}}
\newcommand{\cq}{\mbox{''}}
\newcommand{\bi}[1]{\textit{\textbf{#1}}}
%\newcommand{\vtxt}[2]{ \rotatebox{90}{ \begin{tabular}{p{#1}} \centering{#2} \end{tabular} } }
\newcommand{\vtxt}[2]{ \rotatebox{90}{ \centering{#2} } }

\newcommand{\vgap}{\vspace{0.3cm}}
\newcommand{\m}[1]{\mathscr{#1}}
\newcommand{\M}{\textsf{M}}
\newcommand{\dbsp}{\textsf{D-BSP}}
\newcommand{\bfm}[1]{\mbox{\boldmath $#1$}}
\def\phead#1{~\\\noindent{\bf{#1.}}}
\newcommand{\embox}{\mbox{\hspace*{1em}}}
\newcommand{\para}[1]{\vspace{0.1cm}\noindent{\bf{\boldmath{#1}}}}
\newcommand{\vitem}{\vspace{-0.3cm}\item}
\newcommand{\codesize}{\scriptsize}
\newcommand{\codewidth}{0.98\textwidth}
\newcommand{\codeindent}{-0.8cm}

\newcommand{\fnc}[1]{\textrm{\bf{\sc{#1}}}}
\newcommand{\TBL}[2]{\begin{tabular}{@{} #1 @{}} #2 \end{tabular}}
\newcommand{\ft}[1]{\footnotesize #1}
\newcommand{\T}{\hspace{1em}}

% math notations
\newcommand{\R}{\ensuremath{\mathbb R}}
\newcommand{\Z}{\ensuremath{\mathbb Z}}
\newcommand{\N}{\ensuremath{\mathbb N}}
%\newcommand{\F}{\ensuremath{\mathcal F}}
\newcommand{\SymGrp}{\ensuremath{\mathfrak S}}

\def\comment#1{\hfill{\color{gray}{$\left\{\textrm{{\em{#1}}}\right\}$}}}
\def\lcomment#1{\hfill{\color{gray}{$\left\{\textrm{{\em{#1}}}\right.$}}}
\def\rcomment#1{\hfill{\color{gray}{$\left.\textrm{{\em{#1}}}\right\}$}}}
\def\fcomment#1{\hfill{\color{gray}{$\textrm{{\em{#1}}}$}}}
\def\func#1{\textrm{\bf{\sc{#1}}}}
\def\funcbf#1{\textrm{\textbf{\textsc{#1}}}}


% asymptotic notations
\newcommand{\Oh}[1]{{\mathcal O}\left({#1}\right)}
\newcommand{\LOh}[1]{{\mathcal O}\left({#1}\right.}
\newcommand{\ROh}[1]{{\mathcal O}\left.{#1}\right)}
\newcommand{\oh}[1]{{o}\left({#1}\right)}
\newcommand{\Om}[1]{{\Omega}\left({#1}\right)}
\newcommand{\om}[1]{{\omega}\left({#1}\right)}
\newcommand{\Th}[1]{{\Theta}\left({#1}\right)}

\newcommand{\xif}{{\bf{{if~}}}}
\newcommand{\xthen}{{\bf{{then~}}}}
\newcommand{\xelse}{{\bf{{else~}}}}
\newcommand{\xelseif}{{\bf{{elif~}}}}
\newcommand{\xfi}{{\bf{{fi~}}}}
\newcommand{\xfor}{{\bf{{for~}}}}
\newcommand{\xeach}{{\bf{{each~}}}}
\newcommand{\xto}{{\bf{{to~}}}}
\newcommand{\xdownto}{{\bf{{downto~}}}}
\newcommand{\xby}{{\bf{{by~}}}}
\newcommand{\xdo}{{\bf{{do~}}}}
\newcommand{\xrof}{{\bf{{rof~}}}}
\newcommand{\xwhile}{{\bf{{while~}}}}
\newcommand{\xendwhile}{{\bf{{endwhile~}}}}
\newcommand{\xrepeat}{{\bf{{repeat~}}}}
\newcommand{\xuntil}{{\bf{{until~}}}}
\newcommand{\xand}{{\bf{{and~}}}}
\newcommand{\xor}{{\bf{{or~}}}}
\newcommand{\xerror}{{\bf{{error~}}}}
\newcommand{\xprint}{{\bf{{print~}}}}
\newcommand{\xreturn}{{\bf{{return~}}}}
\newcommand{\xpfor}{{\bf{{pfor~}}}}
\newcommand{\xnil}{\textrm{\sc{nil}}}
\newcommand{\xparallel}{{\bf{{parallel:~}}}}
\newcommand{\xparallelfor}{{\bf{{parallel~for~}}}}
\newcommand{\xpar}{{\bf{{par:~}}}}
\newcommand{\xblank}{{$\phantom{aimmd}$}}
\newcommand{\xblankpar}{{$\phantom{par:}$}}
\newcommand{\xspawn}{{\bf{\em{spawn~}}}}
\newcommand{\xsync}{{\bf{\em{sync~}}}}
\newcommand{\xcomment}{\hfill $\rhd$ }
%\newcommand{\T}{\hspace{0.3cm}}

\newcommand{\mfunc}[1]{\mathcal{#1}}
\newcommand{\MM}[1]{\mfunc{MM}#1}
\newcommand{\idp}{$\mathcal{I}$-$\m{DP}$}
\newcommand{\lalgo}{$\mathcal{I}$}
\newcommand{\rdp}{$\mathcal{R}$-$\m{DP}$}
\newcommand{\calgo}{$\mathcal{R}$}
\newcommand{\autogen}{$\textsc{Autogen}$}
\newcommand{\fracdp}{$\m{FRACTAL}$-$\m{DP}$}

\newcommand{\nvs}{\vspace{-0.15cm}}
\newcommand{\vsitem}{\vspace{-0.15cm}\item}

% to add new commands to algorithmic environment
\makeatletter
\newcommand{\ALOOP}[1]{\ALC@it\algorithmicloop\ #1%
  \begin{ALC@loop}}
\newcommand{\ENDALOOP}{\end{ALC@loop}\ALC@it\algorithmicendloop}
\newcommand{\algorithmicinput}{\textbf{Input:}}
\newcommand{\INPUT}{\item[\algorithmicinput]}
\newcommand{\algorithmicoutput}{\textbf{Output:}}
\newcommand{\OUTPUT}{\item[\algorithmicoutput]}
\newcommand{\algorithmicinvoke}{\textbf{Invoke:}}
\newcommand{\INVOKE}{\item[\algorithmicinvoke]}
\makeatother

%\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\definecolor{gray}{rgb}{0.3,0.3,0.3}
\colorlet{lightblue}{blue!15}
\colorlet{lightred}{red!20}
\colorlet{lightyellow}{green!20}
\colorlet{framecolor}{yellow!20}
\colorlet{frameloopcolor}{yellow!20}
\colorlet{algocolor}{orange!20}

\surroundwithmdframed[
  backgroundcolor   = algocolor,
  hidealllines      = true,
  innerleftmargin   = 0.5em,
  innerrightmargin  = 0.5em,
  innertopmargin    = -1.1em,
  innerbottommargin = 0em,
  leftline=true,
  rightline=true,
  bottomline=true,
  topline=true,
  skipabove         = .5\baselineskip,
  skipbelow         = .5\baselineskip
]{algorithm}

\newcommand{\parll}{\textbf{par:} }
\newcommand{\phantomparll}{\phantom{\textbf{par: } }}

\makeatletter
   \newcommand\figcaption{\def\@captype{figure}\caption}
   \newcommand\tabcaption{\def\@captype{table}\caption}
\makeatother

%--------------- TCOLORBOX -------------------
% \colorlet{algotitlebarcolor}{green!20}
% \colorlet{algotitlebarcolortop}{green!40}
% \colorlet{algotitlebarcolorbottom}{green!20}
% \colorlet{framecolor}{yellow!20}
% \colorlet{framecolortop}{yellow!40}
% \colorlet{framecolorbottom}{yellow!20}
\colorlet{algotitlebarcolor}{gray!20}
\colorlet{algotitlebarcolortop}{gray!40}
\colorlet{algotitlebarcolorbottom}{gray!20}
\colorlet{framecolor}{white!20}
\colorlet{framecolortop}{white!40}
\colorlet{framecolorbottom}{white!20}
\colorlet{bluetop}{cyan!40}
\colorlet{bluebottom}{cyan!20}
%\colorlet{redtop}{RubineRed!40}
%\colorlet{redbottom}{RubineRed!20}
\colorlet{greentop}{green!40}
\colorlet{greenbottom}{green!20}
\colorlet{shadowcolor}{gray}
\colorlet{algotitlecolor}{black}
\colorlet{algoframecolor}{gray}
\colorlet{tabletitlecolor}{gray!30}
\colorlet{tablealtrowcolor}{gray!15}
\colorlet{tablefillcolor}{white!40}
\colorlet{tablefillcolor2}{white!20}

\newtcolorbox{mycolorbox}[1]
{skin=enhanced,colbacktitle=algotitlebarcolor,coltitle=algotitlecolor,colback=algocolor,colframe=algoframecolor,title style={top color=algotitlebarcolortop, bottom color=algotitlebarcolorbottom},interior style={top color=framecolortop, bottom color=framecolorbottom},drop shadow,title={\codesize #1}}

\newcommand{\algotopspace}{\vspace{-0.35cm}}
\newcommand{\algomiddlespace}{\vspace{0.1cm}}
\newcommand{\algobottomspace}{\vspace{-0.15cm}}
\newcommand{\algodiffspace}{\vspace{-0.15cm}}
\newcommand{\algoinput}{{\bf{{Input:~}}}}
\newcommand{\algooutput}{{\\\bf{{Output:~}}}}
\newcommand{\algorequire}{{\\\bf{{Require:~}}}}

%--------------- TABLE COLOR ---------------
\arrayrulecolor{gray}
\setlength{\arrayrulewidth}{0.4mm}
\renewcommand{\arraystretch}{0.8}
\newsavebox{\tablebox}
\NewEnviron{colortabular}[1]{%
  \addtolength{\extrarowheight}{1ex}%
%  \rowcolors{2}{tablefillcolor}{tablefillcolor2}
  \savebox{\tablebox}{%
    \begin{tabular}{#1}%
	  \rowcolor{tabletitlecolor}
      \BODY%
    \end{tabular}}
  \begin{tikzpicture}
    \begin{scope}
      \clip[rounded corners=1ex] (0,-\dp\tablebox) -- (\wd\tablebox,-\dp\tablebox) -- (\wd\tablebox,\ht\tablebox) -- (0,\ht\tablebox) -- cycle;
      \node at (0,-\dp\tablebox) [anchor=south west,inner sep=0pt]{\usebox{\tablebox}};
    \end{scope}
    \draw[rounded corners=1ex] (0,-\dp\tablebox) -- (\wd\tablebox,-\dp\tablebox) -- (\wd\tablebox,\ht\tablebox) -- (0,\ht\tablebox) -- cycle;
  \end{tikzpicture}
}

\newcommand{\MinLaserConvexArea}{{\sc MinLaser-ConvexArea}\xspace}
\newcommand{\Att}[1]{\textcolor{red}{#1}}
\newcommand{\csaba}[1]{\textcolor{blue}{Csaba: #1}}
\newcommand{\rathish}[1]{\textcolor{purple}{Rathish: #1}}
\newcommand{\joe}[1]{\textcolor{olive}{Joe: #1}}
\newcommand{\jie}[1]{\textcolor{magenta}{Jie: #1}}

\newcommand{\area}{{\rm area}}
\newcommand{\conv}{{\rm conv}}
\newcommand{\diam}{{\rm diam}}
\newcommand{\per}{{\rm per}}
\newcommand{\len}{{\rm len}}
\newcommand{\opt}{{\rm OPT}}
\newcommand{\alg}{{\rm ALG}}

\newcommand{\denselist}{\itemsep 0pt\parsep=1pt\partopsep 0pt}
\newcommand{\bitem}{\begin{itemize}\denselist}
	\newcommand{\eitem}{\end{itemize}}
\newcommand{\benum}{\begin{enumerate}\denselist}
	\newcommand{\eenum}{\end{enumerate}}



==> min-diameter-k-laser-short.tex <==
\subsection{$O(1)$-Approximation for \md in Simple Polygons}
\label{sec:k-laser-mindiameter-short}
Using the bi-criteria algorithm from the previous section we obtain an $O(1)$-approximation for \md; see Appendix~\ref{sec:k-laser-mindiameter-full} for details.% (in Section~\ref{sec:polygon-holes} we use the same idea to get an $O(1)$-approximation for \md in polygons with holes). 

==> min-laser-diameter-short.tex <==
\subsection{Bi-Criteria Approximation for Diameter}\label{sec:minlaser-diameter-short}
By cutting \P with a grid of lasers spaced \d apart (and then carefully removing some lasers), we partition the polygon into pieces of diameter $O(\d)$ using $O(k^*)$ lasers where $k^*$ is the minimum number of lasers required to get diameter \d; see Appendix~\ref{sec:minlaser-diameter-full} for details.






==> open-problems.tex <==
\section{Open questions}
\subsection{Approximation results for polygon with holes}
At present, all our hardness results are on polygon with holes. Hence, we want some approximation results for them.

\begin{enumerate}
	\item Given a polygon with holes and a diameter budget $\delta$, minimize the number of general directional lasers to cut the polygon satisfying the cell diameter budget.
	
	We are hoping for a $O(\log n)$ approximation.
	
	\item Given a polygon with holes and a diameter budget $\delta$, minimize the number of orthogonal lasers to cut the polygon satisfying the cell diameter budget.
	\textbf{\rathish{I think we discussed a bi-criteria algorithm for this version. Need to verify.}}
	
	\item Given a polygon with holes and an area budget $\delta$, minimize the number of general directional lasers to cut the polygon satisfying the cell area budget.
	
	\item Given a polygon with holes and an area budget $\delta$, minimize the number of orthogonal lasers to cut the polygon satisfying the cell area budget.
	
\end{enumerate}

\subsection{Hardness results for simple polygon}
Either show that the problems are hard in simple polygons or give exact algorithms.


==> orthogonal-laser-short.tex <==
\section{Axis-Parallel Lasers}
\label{sec:orthogonal-laser}

In this section we study \mld and \mla under the constraint that all lasers must be axis-parallel (the edges of \P may have arbitrary orientations). The algorithms for both problems start with a ``window partitioning'' \P into ``(pseudo-)histograms'' of stabbing number at most three, and are then tuned to the specific measures to partition the histograms. We use a simple sweepline algorithm for the diameter, and a dynamic program for the area. The main result is:
\begin{theorem}\label{thm:minlaser-measure-axis-paralleli}
Let \P be a simple polygon with $n$ vertices and let $k^*$ be the minimum number of axis-parallel lasers needed to subdivide $P$ into pieces of area (diameter) at most $1$.
There is an algorithm that finds $O(k^*)$ axis-parallel lasers that subdivide \P into pieces of area (diameter) at most $1$ in time polynomial in $n$ and $\area(\P)$ ($\diam(\P)$).
\end{theorem}

\subsection{Reduction to Histograms}
\label{ssec:window}

A \emph{histogram} is a simple polygon bounded by an axis-parallel line segment, the \emph{base}, and an $x$- or $y$-monotone polygonal chain between the endpoints of the base.

The \emph{window partition} of a simple polygon was originally used for the design of data structures that support link distance queries~\cite{LinkDistance,Suri90}. In this section, we use the axis-parallel version, which partitions a simple polygon $P$ into histograms such that every axis-parallel chord of $P$ intersects at most 3 histograms. Window partitions for orthogonal polygons can be computed by a standard recursion~\cite{LinkDistance,Suri90}; we use a modified version where we recurse until the remaining subpolygons are below the size threshold $1$. This modification guarantees termination on all simple polygons (not only orthogonal polygons).

\begin{figure*}[!ht]
	\centering
	\includegraphics[scale=1]{window-partition.pdf}
	\caption{Window partition of a polygon $Q$ with a horizontal base $b$ into a maximal histogram $H$ (colored gold) and four polygons $Q_1$, $Q_2$, $Q_3$, and $Q_4$ (in white). If the sizes (areas/diameters) of $Q_1$, $Q_2$, $Q_3$, and $Q_4$ are each at most $1$, then $Q$ is a  pseudo-histogram.}
	\label{fig:window}
\end{figure*}

\smallskip\noindent\textbf{Window Partition Algorithm.}
Given a simple polygon \P, let $b$ be an axis-parallel chord of \P that subdivides \P into two simple polygons $P_1$ and $P_2$ with a common base $b$. Let $\mathcal{S}=\{(P_1,b),(P_2,b)\}$ be a set of tuples where each tuple has a polygon and its axis-parallel base, and let $\mathcal{H}=\emptyset$ be the set of histograms. While $\mathcal{S}$ contains a pair $(Q,b)$, where the size (e.g., the diameter)
of $Q$ is more than 1, do the following:
\benum
\item compute the maximal histogram\footnote{Without loss of generality, assume $b$ is horizontal. $H$ can be obtained by taking all points of $Q$ reachable through a vertical line from points on $b$.} $H$ of base $b$ in $Q$, and add $(H,b)$ to $\mathcal{H}$; See Figure~\ref{fig:window}.
\item update $\mathcal{S}$ by replacing $(Q,b)$ with the pairs $(Q_i,b_i)$, where the polygons $Q_i$ are the connected components of $Q\setminus H$, and $b_i$ is the boundary between $Q_i$ and $H$.
\eenum
Return $\mathcal{H}$ and $\mathcal{S}$.


\paragraph{Pseudo-histograms.}
%\csaba{We should change $\diam$ to ``measure'' that can be area, diameter, or inradius.}\val{said "e.g., diam" in the previous para}
Let $T_1$ and $T_2$ be the recursion trees of the algorithm, rooted at $P_1$ and $P_2$, respectively. Let $T=T_1\cup T_2$. Each node $v\in T$ corresponds to a polygon $Q_v\subset P$. Every nonleaf node $v\in T$ also corresponds to a histogram $H_v\subset Q_v$; it is possible that size$(H_v)\leq 1$ but size$(Q_v)>1$ (the size is $\area$ or $\diam$ based on the problem). For a leaf $v\in T$, we have either size$(Q_v)\leq 1$, or $H_v=Q_v$ and size$(H_v)>1$. The polygons $Q_v$ at leaf nodes and the histograms $H_v$ at nonleaf nodes jointly form a subdivision of $P$.

Every node $v\in T$ in the recursion tree corresponds to a polygon-base pair $(Q_v,b_v)$.
For any subset $U\subset V(T)$, where $V(T)$ is the set of vertices of $T$, the bases $\{b_u:u\in U\}$
decompose $P$ into simply connected cells. For every $u\in U$, there is a cell $P_u$ in the decomposition such that  $H_u\subset P_u\subset Q_u$. Since every axis-parallel chord of $P$ crosses at most 2 bases, it can intersect at most 3 polygons in such a decomposition. %\rathish{I don't understand the importance of a subset of vertices $U$.}\csaba{Each vertex is a cut-vertex in a tree; so a set of vertices decompose a tree into subtrees. Each vertex corresponds to a base (chord of \P), which decompose \P into cells.}

In a bottom-up traversal of $T$, we can find a subset $U\subset V(T)$ such that $\{b_u:u\in U\}$ decomposes
$P$ into polygons $P_u$, $u\in U$, such that size$(P_u)>1$ but the size of every component of $P_u\setminus H_u$ is at most $1$.
Each polygon $P_u$ consists of a histogram $H_u$ with base $b_u$, and subpolygons (\emph{pockets}) of size at most 1 attached to some edges of $H_u$ orthogonal to $b_u$. We call each such polygon $P_u$ a \emph{pseudo-histogram}. See Figure~\ref{fig:window}.

\subsection{$O(1)$-Approximation for \mld}
\label{sec:min-orthogonal-laser-diameter}

We start with an $O(1)$-approximation for histograms, and then extend our algorithm to pseudo-histograms and simple polygons. %Without loss of generality, we assume that the base is horizontal.

\begin{theorem}\label{thm:HistogramDiam}
There is an algorithm that, given a histogram $P$ with $n$ vertices, computes an $O(1)$-approximation for the axis-parallel \mld problem in time polynomial in $n$ and $\diam(P)$.
\end{theorem}
\begin{proof}
We place a raster of vertical lasers, equally spaced at distance 1/2 apart; and then use a sweepline algorithm to place horizontal lasers at ``critical'' points. A charging scheme shows that the lasers placed by the algorithm can be charged to the lasers of $\opt$ such that each laser in $\opt$ is charged at most $O(1)$ times. See Appendix~\ref{app:min-orthogonal-laser-diameter} for further details.
\end{proof}

An adaptation of the sweepline algorithm in the proof of Theorem~\ref{thm:HistogramDiam} can also find an $O(1)$-approximation for \mld in a pseudo-histogram (see further details in Appendix~\ref{app:min-orthogonal-laser-diameter}). As noted above, each laser intersects at most 3 pseudo-histograms, hence the union of lasers in the solutions for pseudo-histograms is an $O(1)$-approximations for \mld $P$. This proves the diameter part of Theorem~\ref{thm:minlaser-measure-axis-paralleli}.

%\val{commented out this thm since it's part of thm:minlaser-measure-axis-parallel now}\begin{theorem}\label{thm:SimPolygon-OrthogonalLasers}There is an algorithm that, given a simple polygon $P$ with $n$ vertices,computes an $O(1)$-approximation for the axis-parallel \mld problem in time polynomial in $n$ and $\diam(P)$.\end{theorem}


\subsection{Discretization of Solution Space in a Histogram Polygon}
\label{sec:min-orthogonal-laser-DP}

Consider a histogram polygon $P$ having $n$ vertices.
%
We assume that the vertices
are in general position, in the sense that no three vertices are collinear. We
%In this section we
show that there is a discrete set of candidate orthogonal chords such that lasers chosen from this set yield an $O(1)$ approximation for minimizing the number of lasers, subject to a target measure bound $1$ on the obtained pieces. This is useful for finding an $O(1)$ approximation for \mla by dynamic programming.

%Let $H_P$ be the set of horizontal chords in $P$ having at least one of its endpoints at a vertex of $P$; such horizontal chords yield the \emph{horizontal decomposition} of $P$ into horizontal trapezoids (which are rectangles if $P$ is orthogonal).  Let $V_P$ be the set of vertical chords in $P$ having top endpoint at a vertex of $P$; such vertical chords yield the \emph{vertical decomposition} of $P$ into vertical trapezoids (which are rectangles if $P$ is orthogonal).


%, to be described in the next subsection.

We prove the following lemma in Appendix~\ref{app:discretization}, which extends to pseudo-histograms.

\begin{lemma}%\label{lem:cl-area}
For a histogram $P$, let $k^*$ be the minimum number of axis-parallel lasers that subdivide
$P$ into pieces of area (diameter) at most 1. We can find a set $C$ of $O(n+\area(P))$ ($O(n+\text{per}(P))$) chords of $P$,
such that $O(k^*)$ lasers from $C$ can subdivide $P$ into pieces of area (diameter) at most 1.
\end{lemma}


\subsection{$O(1)$-Approximation for \textbf{MinLaser-Area}}
\label{sec:min-orthogonal-laser-area}

We now consider the \mla with axis-parallel lasers chosen
from a discrete set to achieve pieces of area at most $1$.
An $O(1)$-approximation algorithm is based on the window partition method
described earlier, allowing us to reduce to the case of subdividing a
pseudo-histogram, for which we give a dynamic program
to choose lasers from the discrete candidate set.
In Appendix~\ref{app:min-orthogonal-laser-DP}, we describe the algorithm using area as the measure.
With slight modifications, the algorithm also applies to the measure of
diameter, allowing us to solve \mld in pseudo-histograms
(albeit in a higher polynomial time bound than stated in Theorem~\ref{thm:HistogramDiam}).

%\val{commented out since it's now stated in the begnnning of the section }\begin{theorem}\label{thm:minlaser-measure-axis-parallel}Let \P be a simple polygon with $n$ vertices and let $k^*$ be the minimum number of axis-parallel lasers needed to subdivide $P$ into pieces of area (diameter) at most $1$.There exists an algorithm that returns $O(k^*)$ axis-parallel lasers that subdivide \P into pieces of area (diameter) at most $1$ in time polynomial in $n$ and $\area(\P)$ ($\diam(\P)$).\end{theorem}


==> polygon-holes-short.tex <==
\section{Diameter Measure in Polygons with Holes and Axis-Parallel Lasers}
\label{sec:polygon-holes}

%\subsection{Bi-Criteria Approximation for Diameter}\label{sec:bicriteria-holes}
Our next theorem (proof in Appendix~\ref{sec:bicriteria-holes}) gives a bi-criteria approximation for the diameter version
in a polygon with holes when lasers are constrained to be axis-parallel.
The approach is similar to the algorithm for simple polygons
and lasers of arbitrary orientations (cf.~Section~\ref{sec:minlaser-diameter-short}) in that both use grid lines, but they differ significantly to handle holes in a polygon when the lasers are axis-parallel. Particularly, in simple polygons we place lasers along grid lines, while in polygons with holes the grid lines just divide the problem into sub-problems.

\begin{theorem}\label{thm:bicriteria-diam-holes}
	Let $P$ be a polygon with holes of diameter ${\rm diam}(P)$ having $n$ vertices,
	and let $k^*$ be the minimum number of laser cuts that partition $P$
	into pieces each of diameter at most $\delta$ for a fixed $\delta>0$. In time
	polynomial in $n$ and ${\rm diam}(P)/\delta$, one can compute a set of
    at most $6k^*$ lasers that subdivide $P$ into pieces each of diameter
	at most $2^{3/2}\delta$.
\end{theorem}


Similarly to Section~\ref{sec:k-laser-mindiameter-short}, we can use the bi-criteria algorithm to
derive a constant-factor approximation for minimizing the maximum diameter of a cell in the arrangement of a given number \k of axis-parallel lasers. Our $O(1)$-approximation algorithm  (Theorem~\ref{thm:approx-k-laser-diam-hole}, proof in Appendix~\ref{sec:constant-holes})
 repeatedly decreases the $x$- and $y$- separation in the bi-criteria solution from Theorem~\ref{thm:bicriteria-diam-holes} until the number of placed lasers is about to jump over 6\k; then, the number of lasers is decreased by a factor of $6$ while increasing the diameter by a constant factor.

\begin{theorem}\label{thm:approx-k-laser-diam-hole}%Let $P$ be a simple polygon with $n$ vertices, and
Let $\delta^*$ be the minimum diameter achievable with $k$ axis-parallel lasers.
For every $\epsilon>0$, one can compute a set of at most $k$ axis-parallel lasers that partition $P$ into pieces each of diameter at most $12\sqrt{2}(1+\epsilon)\d^*$ in time polynomial in $n$, ${\rm diam}(P)/\delta^*$, and $\epsilon$.
\end{theorem}

